Simultaneous Locomotion Mode Classification and Continuous Gait Phase Estimation for Transtibial Prostheses

Recognizing and identifying human locomotion is a critical step to ensuring fluent control of wearable robots, such as transtibial prostheses. In particular, classifying the intended locomotion mode and estimating the gait phase are key. In this work, a novel, interpretable, and computationally efficient algorithm is presented for simultaneously predicting locomotion mode and gait phase. Using able-bodied (AB) and transtibial prosthesis (PR) data, seven locomotion modes are tested including slow, medium, and fast level walking (0.6, 0.8, and 1.0 m/s), ramp ascent/descent (5 degrees), and stair ascent/descent (20 cm height). Overall classification accuracy was 99.1$\%$ and 99.3$\%$ for the AB and PR conditions, respectively. The average gait phase error across all data was less than 4$\%$. Exploiting the structure of the data, computational efficiency reached 2.91 $\mu$s per time step. The time complexity of this algorithm scales as $O(N\cdot M)$ with the number of locomotion modes $M$ and samples per gait cycle $N$. This efficiency and high accuracy could accommodate a much larger set of locomotion modes ($\sim$ 700 on Open-Source Leg Prosthesis) to handle the wide range of activities pursued by individuals during daily living.

==> 02_Methods.tex <==
Perhaps section II.A should occur at the end of section II?
\subsection{Locomotion Data}

\begin{comment}
    

there are 6 signals coming in: R/L Thigh/Shank/Foot
foot used for ground truth gait detection
several activities:
- slow walking
- med walking
- fast walking
- ramp ascent
- ramp descent
- stair ascent
- stair descent
\end{comment}

% Include an image showing all activities with AB on top row and Bypass on bottom row.

\subsubsection{Data Collection}

To evaluate the locomotion classification, gait phase estimation, and computational reduction approaches proposed herein, data was collected and processed for later offline analysis. Two datasets were collected; the first from a single able-bodied (AB) individual (180 cm height, 75 kg mass), and the second from that same individual walking on a unilateral transtibial robotic prostheses (PR), namely the version 1 Open-Source Leg (OSL)~\cite{azocar2018design} via a bypass adapter. Figure X shows these two conditions, along with the locomotion modes that were selected for identification, which are level treadmill walking (at 0.6, 0.8, and 1.0 m/s), fixed ramp ascent and descent (5-degree slope, X m length), and stair ascent and descent (X cm stair height, X steps). When walking with the prosthesis, a passive controller was employed, defined by constant ankle impedance parameters of 0 degrees equilibrium angle, 0.09 Nm/deg/kg stiffness, and 0.075 Nms/deg/kg damping, intended to approximate the behavior of a passive ankle-foot prosthesis. A contralateral shoe lift was donned to accommodate leg length difference from the adapter.

For all conditions, the individual wore the XSENS MVN Link motion capture suit for real-time measurement of the right and left global thigh ($\theta_{th-r}$ and $\theta_{th-l}$), shank ($\theta_{sh-r}$ and $\theta_{sh-l}$), and foot angles ($\theta_{f-r}$ and $\theta_{f-l}$, respectively). Only the four angles of the bilateral thigh and shank serve as inputs to the locomotion classification and phase estimation algorithm, while the bilateral foot angles were used strictly for heel strike (HS) identification (~\ref{sec:processing}). The XSENS suit was calibrated following the standard calibration procedure provided within the XSENS Analyze software, and the suit communicated to a Raspberry Pi wirelessly via a private Wi-Fi router for data logging. The system operated at approximately 230 Hz, bounded by the XSENS communication frequency. 

\subsubsection{Data Processing}
\label{sec:processing}

For both AB and PR conditions, two minutes of steady-state walking data were collected at each treadmill speed, 10 trials of ramp ascent/descent, and 5 trials of stair ascent/descent. The step-to-step gait was employed for PR stair descent, as is commonly recommended by clinicians [], while the step-over-step gait was used for PR stair ascent and AB stair ascent/descent, highlighting the ability of this approach to be used for a wide range of gait types. The data were then split into training data and evaluation data (details in Tables~\ref{tb:AB_Data} and~\ref{tb:PR_Data}). In level-ground and ramp walking, right-side (or prosthesis-side) HS was identified by peaks in $\theta_{f-r}$ [], while peaks in $\theta_{sh-r}$ were used during stair ascent and descent and manually verified. HS identification was only used to calibrate the training data and to serve as ground truth gait phase (defined as normalized time between each HS) for the evaluation data.
%
\begin{figure*}[t!]
    \centering
    \includegraphics[width = 0.8\linewidth, trim={0cm 16.6cm 0cm 0cm},clip]{Figures/Data_Collection.pdf}
    \caption{Experimental data was collected from 7 different locomotion modes: slow/medium/fast walking, ramp ascent/descent, and stair ascent/descent), with 2 different conditions: able-bodied (AB) and with the OpenSource Leg (OSL) transtibial prostheses (PR).} 
	\label{fig:Data_Collection}
\end{figure*}
%
%
%
%
%
%
\subsection{Locomotion Classification and Gait Phase Estimation}

\subsubsection{System Overview}

An overview of the system architecture is shown in Fig. X. The overall control framework takes as input the current global thigh and shank angles ($\theta_{th-r}$, $\theta_{th-l}$, $\theta_{sh-r}$, and $\theta_{sh-l}$), and outputs the predicted locomotion mode and the corresponding estimate of the gait phase progression for that mode. Using the training data, a baseline trajectory for each locomotion mode (referred to herein as a kernel) is identified. At each time instant thereafter, each kernel is compared to the most recent historical data, and the kernel with the best matching is selected as the predicted locomotion mode. The phase shift of that kernel that results in the best overall matching is used to estimate the gait phase progression. Note that this process considers kernel matching for all four segment angles, while Fig. X shows only $\theta_{th-r}$.

%
%
%
%
\begin{table}[b!]
\centering
\caption{Data collection summary with able-body (ab)}
\label{tb:AB_Data}
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{000000} 
{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Locomotion \\ Mode \\ (m)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Data\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Evaluation \\ Data\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Kernel \\ Size \\ $(N_m)$\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Kernel \\ Resolution \\ {[}gait \%{]}\end{tabular}}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
Slow & 12750 & 12750   & 392  & 0.26             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Med  & 13000 & 13000   & 313  & 0.32             \\ \hline
\rowcolor[HTML]{FFFFFF} 
Fast & 13000 & 13000   & 280  & 0.36             \\ \hline
\rowcolor[HTML]{FFFFFF} 
RA   & 5678  & 3100    & 283  & 0.35             \\ \hline
\rowcolor[HTML]{FFFFFF} 
RD   & 5724  & 4183    & 286  & 0.35             \\ \hline
\rowcolor[HTML]{FFFFFF} 
SA   & 3820  & 2636    & 318  & 0.31             \\ \hline
\rowcolor[HTML]{FFFFFF} 
SD   & 3714  & 1475    & 309  & 0.32             \\ \hline
\end{tabular}
\end{table}
%
%
%
%

\subsubsection{Steady-State Kernel Generation}

Steady-state kernels for each locomotion mode and each segment angle are generated offline using the training data. Once the data are segmented into strides, the average thigh and shank angle trajectories as a function of gait phase are stored as kernels. Unlike neural-network-based algorithms, this model-based training requires only a small number of steady-state strides ($\sim$ 10) from the individual and is computationally light. In theory, only a single steady-state stride could be used to generate each kernel, though increasing the number of strides can lead to more robust predictions by averaging out the variance from individual strides. Seven kernels are generated representing the seven locomotion modes (three level walking speeds, ramp ascent/descent, and stair ascent/descent), with each kernel containing segment angle trajectories (bilateral thigh and shank).

\begin{figure*}[t!]
    \centering
    \includegraphics[width = 0.8\linewidth, trim={0cm 24cm 0cm 0cm},clip]{Figures/intro_figure.pdf}
    \caption{A window of historical data is compared to sliding locomotion mode kernels. Locomotion modes include slow/medium/fast walking (Slow, Med, Fast), ramp ascent/descent (RA, RD), and stair ascent/descent (SA, SD). The kernel with the lowest sum of squares error (SSE) is selected as the current locomotion mode (shown as SA, SSE = 2), and the sliding configuration that results in that minimum SSE determines the gait phase (shown as $\phi = 30\%$).} 
	\label{fig:Schematic}
\end{figure*}

\subsubsection{The Algortihm...?}

%
%
%
%
\begin{table}[b!]
\centering
\caption{Data collection summary with prosthesis (pr)}
\label{tb:PR_Data}
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{000000} 
{\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Locomotion \\ Mode \\ (m)\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Data\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Evaluation \\ Data\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Kernel \\ Size \\ $(N_m)$\end{tabular}}} & {\color[HTML]{FFFFFF} \textbf{\begin{tabular}[c]{@{}c@{}}Kernel \\ Resolution \\ {[}gait \%{]}\end{tabular}}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
Slow           & 13000 & 13000   & 418            & 0.24                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
Med            & 13500 & 13500   & 343            & 0.29                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
Fast           & 13500 & 13500   & 318            & 0.31                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
RA             & 6174  & 5526    & 343            & 0.29                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
RD             & 7481  & 6011    & 340            & 0.29                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
SA             & 3838  & 2639    & 426            & 0.23                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
SD             & 10466 & 6133    & 387            & 0.26                       \\ \hline
\end{tabular}
\end{table}
%
%
%
%

For notation, let $k_{m}^{s-x}$ represent the individual kernel for locomotion mode $m$, leg segment $s$ (either $th$ or $sh$ for thigh or shank, respectively), and the leg side $x$ ($x = L$ or $R$ for left/right). Modes of 0.6 m/s level walking, 0.8 m/s level walking, 1.0 m/s level walking, ramp ascent, ramp descent, stair ascent, and stair descent are indicated by $m =$ Slow, Med, Fast, RA, RD, SA, and SD, respectively. Individual kernel $k_{m}^{s-x}$ is a ($1 \times N_{m}$) vector, where $N_{m}$ is the average number of data points during a stride of locomotion mode $m$ from the training data ( shown in Tables~\ref{tb:AB_Data} and~\ref{tb:PR_Data}). For example, at the approximately 230 Hz sampling rate, $N_{Slow} = 392$, whereas $N_{Fast} = 280$ in the AB condition (Table~\ref{tb:AB_Data}), as the stride duration is decreased with increased speed. We can stack the kernels from the left and right thigh and shank to create a matrix $k_m = [k_{m}^{th-R}, k_{m}^{th-L}, k_{m}^{sh-R}, k_{m}^{sh-L}]^\top$. The kernels are then doubled so that they can be compared to the most recent historical data in a circular sliding manner. This fully defines the full kernel matrix $K_m$, constructed as 
% ($4 \times N_{m}$) matrix defined by

\begin{equation}
    K_m = 
    \begin{bmatrix}
    k_{m}, & k_m
    \end{bmatrix} 
    \in \mathbb{R}^{4 \times 2N_{m}},
\end{equation}

\noindent where the 4 rows contain the doubled kernels for each leg segment. We then construct a state vector or data vector $d_i = [\theta_i^{th-R}, \theta_i^{th-L}, \theta_i^{sh-R}, \theta_i^{sh-L}]^\top \in \mathbb{R}^{4 \times 1}$ that contains the four segment angles for a given time instant $i$. 
To compare $K_m$ to the most recent historical data, we construct a data history matrix 

\begin{equation}
    D_m(t) = 
    \begin{bmatrix}
    d_{t-T_m}, & \cdots, & d_t
    \end{bmatrix} 
    \in \mathbb{R}^{4 \times N_{m}},
\end{equation}

\noindent where $d_t$ is the current time $t$ data vector, and $d_{t-T}$ is the historical data vector that corresponds to the signals measured one previous kernel period ($T_m = N_m+1$). We then compare $D_m(t)$ to $K_m$ via the sum of squares error (SSE) with a sliding window on $K_m$

\begin{eqnarray}
    E_{m}(t, n) = (D_m(t) - {K_m}_{n}^{n+N_m-1})\\
    SSE_{m}(t, n) = sum\{E_{m}(t, n)^\top E_{m}(t, n)\}\\
    \forall n \in \{1, \cdots, N_m\},
\end{eqnarray}

where $E_{m,n}$ is the difference (or error) between $D_m$ and a ($4 \times N_{m}$) sub-matrix of $K_m$, with only columns $n$ to $n+N_m-1$ considered for each $n$ sliding window iteration. The vector $SSE_m = [SSE_{m,1}, \cdots, SSE_{m,N_m}]$ contains the SSE comparison between the most recent historical data and all sliding configurations of the kernel corresponding to the locomotion mode $m$. The best matching window between $D_m$ and $K_m$ is given by the index of min($SSE_m$). This is repeated for all locomotion modes ($m = \{Slow, Med, Fast, RA, RD, SA, SD\}$), and the locomotion mode with the lowest min($SSE_m$) is selected as the predicted locomotion mode $m^*$. Once the locomotion mode is classified, the index of min($SSE_{m^*}$), which exists between 1 and $N_{m^*}$ is normalized by $N_{m^*}$ to get the estimated gait phase $\phi \in [0,1]$. Therefore, the resolution at which each locomotion mode can estimate the gait phase is defined by $1/N_m$, allowing locomotion modes with longer stride durations to have finer resolution (Tables~\ref{tb:AB_Data} and~\ref{tb:PR_Data}). 

\subsection{Computational Reduction}

\begin{figure*}[t!]
    \centering
    \includegraphics[width = 0.9\linewidth, trim={0cm 19.8cm 0cm 0cm},clip]{Figures/Matrix_fig.pdf}
    \caption{The sliding kernel matrix $K_m$ is compared to historical data $D_m$ via the sum of squares error (SSE). All calculations can be repeated for each time step, such as time = t (left) and time = t+1 (right), or computation can be significantly reduced by exploiting the many shared computations between subsequent time steps (bottom).} 
	\label{fig:Matrix}
\end{figure*}

At each time instant, the above algorithm calculates the SSE (computationally $\mathcal{O}(N_m)$) for each $N_m$ sliding window configuration and repeats this for $M = 7$ locomotion modes. Therefore, the overall computational cost is $\mathcal{O}(N^2 \times M)$ where $N$ represents the sum of all $N_m, m \in [1,M]$. This algorithm is computationally expensive at each time interval, and the computational cost scales linearly with the number of locomotion modes and quadratically as the data collection frequency increases. For implementation in real time, it is undesirable to reduce the number of locomotion modes that can be predicted and to decrease the data collection frequency. Alternatively, computational cost can also be reduced by exploiting the structure of the matrices used in the algorithm. In particular, many of the individual SSE calculations are repeated in consecutive time steps due to much of the data history remaining the same between consecutive time steps, and all of the kernels remaining unchanged. 


The $K_m$ matrix can be expressed as
\begin{eqnarray}
    K_m = [k_m(1), \cdots, k_m(N_m), k_m(1), \cdots, k_m(N_m)]
    % D_m = [d_{t-T}, d_{t-T+1}, \cdots, d_{t-1}, d_t]
\end{eqnarray}

\noindent where each $k_m(n)$ is the $n$th column of the $k_m$ matrix. 
% index  = [K_m^{th-R}, K_m^{th-L}, K_m^{sh-R}, K_m^{sh-L}]_n^\top$ is a ($4 \times$ 1) column vector containing the $n$th elements of the individual kernals $K_m^{s-x}$, and each $d_i = [d_i^{th-R}, d_i^{th-L}, d_i^{sh-R}, d_i^{sh-L}]^\top$ is the ($4 \times$ 1) column vector containing the incoming data for time $i$. 
Temporarily omitting the subscript $m$, the $n$th element of the data-kernel comparison results, vector $SSE$, at time $t$ (denoted $SSE({t,n})$), can be written as
\begin{eqnarray}
    e_1 = (d_{(t-N+1)} - k(n-1)) \label{eq.e1}\\
    e_2 = (d_{t} - k(n-1)) \label{eq.e2}\\
    SSE_{(t,n)} = SSE_{(t-1,n-1)} - \sum e_1^\top e_1 + \sum e_2^\top e_2 \label{eq.sse_n}\\
    e_3 = (d_{(t-N+1)} - k(N)) \label{eq.e3}\\
    e_4 = (d_{t} - k(N)) \label{eq.e4}\\
    SSE_{(t,1)} = SSE_{(t-1,N)} - \sum e_3^\top e_3 + \sum e_4^\top e_4. \label{eq.sse_1}
\end{eqnarray}


% At time instant $t$, let $K_{m}^{s-x}$ be a theoretical locomotion mode kernal of size ($1 \times 3$), meaning that $N_m = 3$. This kernal could be written out as

% \begin{equation}
%     K_{m}^{s-x} = [k_1^{s-x}, k_2^{s-x}, k_3^{s-x}]
% \end{equation}

% Constructing $K_m$ in this case leads to a ($4 \times 6$) matrix. Considering only a single leg segment and leg side, we temporarily omit the superscript of $s-x$ and subscript $m$ to have

% \begin{equation}
%     K = [k_1, k_2, k_3, k_1, k_2, k_3]
% \end{equation}

% \noindent where $k_n$ is the $n$th index of the individual kernel. Calculating the SSE between this $K$ and the corresponding data history $D = [d_{t-2}, d_{t-1}, d_{t}]$, we have

% \begin{eqnarray}
%     SSE_{t.1} = (d_{t-2} - k_1)^2 + (d_{t-1} - k_2)^2 + (d_{t} - k_3)^2\\
%     SSE_{t.2} = (d_{t-2} - k_2)^2 + (d_{t-1} - k_3)^2 + (d_{t} - k_1)^2\\
%     SSE_{t.3} = (d_{t-2} - k_3)^2 + (d_{t-1} - k_1)^2 + (d_{t} - k_2)^2
% \end{eqnarray}

% \noindent where $SSE_{t.n}$ is the scalar SSE calculated for time $t$ and sliding window $n$. Observing time at $t+1$ yields

% \begin{eqnarray}
%     SSE_{t+1.1} = (d_{t-1} - k_1)^2 + (d_{t} - k_2)^2 + (d_{t+1} - k_3)^2\\
%     SSE_{t+1.2} = (d_{t-1} - k_2)^2 + (d_{t} - k_3)^2 + (d_{t+1} - k_1)^2\\
%     SSE_{t+1.3} = (d_{t-1} - k_3)^2 + (d_{t} - k_1)^2 + (d_{t+1} - k_2)^2.
% \end{eqnarray}

% By comparing the first and second set of equations (use eq numbers), the general form for the total SSE calculation at each time instant $t$ can be constructed as
% %
% \[ \begin{cases} 
%       SSE_{t.1} = SSE_{t-1.N} - (d_{t-N+1} - k_N)^2 + (d_{t} - k_N)^2 \\
%       SSE_{t.n} = SSE_{t-1.n-1} - (d_{t-N+1} - k_{n-1})^2 + (d_{t} - k_{n-1})^2 
%       % & \forall n \neq 1 \\
%    \end{cases} \]

\noindent where Eqs.~\ref{eq.e1}-\ref{eq.sse_n} apply for all $n \neq 1$, and Eqs.~\ref{eq.e3}-\ref{eq.sse_1} when $n = 1$. In this way, the previous algorithm, which had computational cost of $\mathcal{O}(N^2 \times M)$ can now be replicated with mathematical equivalence with only $\mathcal{O}(N \times M)$. This computational reduction algorithm is shown graphically in Fig.~\ref{fig:Matrix}. In practice, the data matrix is initialized to zeros ($D_m(0)$) and $SSE_m$ is initialized as the sum of squares error between $K_m$ and $D_m(0)$. Therefore, the calculations from the reduction method are mathematically equivalent after $N_m$ time steps, at most about 1.85 seconds (one time period $T$ of SA in the PR condition) after data collection begins.

% When data collection begins, the $SSE_m$ vector is initialized by comparing the kernal matrix $K_m$ to an initial data history matrix of zeros $D_{m,0}$ of size ($4 \times N_m$). 



% Insert Table with kernel sizes N and and resolutions X.


\begin{comment}
    

To compare a given kernel to the most recent historical data, we construct a data history vector

Let $t_i$ denote the current time index. 



Locomotion activity classification and gait phase estimation occur together 

kernels for:
- slow walking
- med walking
- fast walking
- ramp ascent
- ramp descent
- stair ascent
- stair descent
- sit to stand
- stand to sit
- sit
- stand

Include a schematic/image articulating the method. 

% \subsection{Gait Phase Estimation}

% Include Histogram of gait percentage error.

\subsection{Computational Reduction?}

Include algorithmic details and computation saving trick.



Here is the approach:

When a new data point comes in,

we backward compare each kernel to the historical data (maintaining the size of the kernel being compared)

we do this for each of the 4 data signals and 11 activities, for a total of 44 comparisons.

For each comparison, we slide the trajectories relative to one another and find the alignment that yields the lowest RMSE.

The sum of RMSE values from the 4 data signals is taken, and the activity mode that generates the lowest RMSE sum is selected as the activity classification

With the activity determined, the index providing the best matching for each of the 4 data signals is taken. An average of these 4 gait percentages can be taken, or we can compare the standard deviation and throw out an outlier if necessary.

At each time instant, we generate an activity classification and a gait phase percentage. We compare this to the ground truth activity and gait percentage in this paper.

Under the hood, at each time instant, we generate an RMSE sum for each activity. This means we also generate an minimum RMSE for each of the 44 trajectories. To find the minumum RMSE for each of the 44 trajectories, we must first find the RMSE for each of the N (size of kernel) kernel shifts.

table with number of training datapoints, training strides, evaluation datapoints, and evaluation strides

joint angle definitions

\end{comment}
